Kernel-as-a-Service: A Serverless Interface to GPUs

Serverless computing has made it easier than ever to deploy applications over scalable cloud resources, all the while driving higher utilization for cloud providers. While this technique has worked well for easily divisible resources like CPU and local DRAM, it has struggled to incorporate more expensive and monolithic resources like GPUs or other application accelerators. We cannot simply slap a GPU on a FaaS platform and expect to keep all the benefits serverless promises. We need a more tailored approach if we want to best utilize these critical resources. In this paper we present Kernel-as-a-Service (KaaS), a serverless interface to GPUs. In KaaS, GPUs are first-class citizens that are invoked just like any other serverless function. Rather than mixing host and GPU code as is typically done, KaaS runs graphs of GPU-only code while host code is run on traditional functions. The KaaS system is responsible for managing GPU memory and schedules user kernels across the entire pool of available GPUs rather than relying on static allocations. This approach allows us to more effectively share expensive GPU resources, especially in multitenant environments like the cloud. We add support for KaaS to the Ray distributed computing framework and evaluate it with workloads including a TVM-based deep learning compiler and a BLAS library. Our results show that KaaS is able to drive up to 50x higher throughput and 16x lower latency when GPU resources are contended.

==> latexmkrc <==
# Settings
$xdvipdfmx = "xdvipdfmx -z 6 -o %D %O %S";

$pdf_mode = 5;
$out_dir = 'build';
@default_files = ( 'paper.tex' );

###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for sharelatex
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    $qpdf //= "/usr/local/bin/qpdf";
    $qpdf = $ENV{QPDF} if defined($ENV{QPDF}) && -x $ENV{QPDF};
    return if ! -x $qpdf; # check that qpdf exists
    $qpdf_opts //= "--linearize --newline-before-endstream";
    $qpdf_opts = $ENV{QPDF_OPTS} if defined($ENV{QPDF_OPTS});
    my $status = system($qpdf, split(' ', $qpdf_opts), "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
    system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
    $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
        system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
    if (-e $rtex_file) {
        do_knitr($rtex_file);
    }
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
    my $file = $_[0];
    my ($name, $path) = fileparse($file);
    pushd($path);
    my $return = system "mpost $name";
    popd();
    return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
        # change directory for a limited scope
        my $orig_dir = cwd();
        my $subdir = dirname($target);
        chdir($subdir);
        # run chktex on main file
        $status = system("/usr/bin/run-chktex.sh", $orig_dir, $file);
        # go back to original directory
        chdir($orig_dir);

        # in VALIDATE mode we always exit after running chktex
        # otherwise we exit if EXIT_ON_ERROR is set

        if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
            # chktex doesn't let us access the error info via exit status
            # so look through the output
            open(my $fh, "<", "output.chktex");
            my $errors = 0;
            {
                local $/ = "\n";
                while(<$fh>) {
                    if (/^\S+:\d+:\d+: Error:/) {
                        $errors++;
                        print;
                    }
                }
            }
            close($fh);
            exit(1) if $errors > 0;
            exit(0) if $ENV{'CHKTEX_VALIDATE'};
        }
    }
}




==> mainSrc/bak_future.tex <==
One of the more important benefits of a heterogeneous cloud function approach like \system{} is the freedom it provides for future innovations. While optimizations for traditional FaaS systems have been well researched, we have argued in this paper that those optimizations are not always appropriate for GPU-enabled FaaS functions. The reality is that a general-purpose function interface does not provide sufficient control or visibility to the system to take advantage of the unique properties of accelerators like GPUs. While our proof-of-concept implementation has demonstrated how these properties could be exploited, they remain relatively na\"ive. In the following sections we discuss what we can learn from these simple techniques and how they might be improved in a more full-featured implementation.

\levelstay{Scheduling Policies}
\label{sec:futScheduling}
The scheduling policies that route requests from clients to \system{} executors provides a rich design space with many tradeoffs. Scheduling in distributed systems is a field that has been studied extensively for decades and there is much to learn from that work. To use the terminology of Ghodsi et. al. (\cite{drf}), our schedulers provide pareto optimality and a sharing incentive (in most cases), but are not envy-free nor strategy-proof. A more sophisticated policy would incorporate information on estimated job runtime and previous allocations to improve performance in all 4 categories of scheduling fairness. Furthermore, the KaaS technique provides insight into data usage patterns which will allow data-aware scheduling or even pre-warming of workloads while scaling. Unlike general-purpose functions, the concept of ``warmness'' in a KaaS system is more continuous and flexible. Code incurs no significant cold-start overheads while function data can be cached at multiple tiers of the storage hierarchy. This property will allow future systems to explore a richer design space of warming policies than is available in current systems.

\levelstay{GPU Compute Resource Sharing}
\label{sec:futCompSharing}
When GPUs are assigned exclusively to functions, it is up to each workload to efficiently utilize the compute resources (i.e. SMs). This can be challenging or impossible for some workloads.
% For example, our resnet50 workload is only capable of using \colorbox{red}{XX\%} of available SMs.
In a KaaS system, we have insight into the compute resource requirements of each workload and can spatially share the GPU among multiple simultaneous requests or exploit intra-request parallelism \jd{This one? It's cited in 7.2}\np{try to remember that TVM? paper that was optimizing the compiler for density rather than raw perf} \cite{rammer}. We may also interleave requests at a kernel-granularity rather than running entire \kfunc{}s to completion to provide more flexible fairness policies.

\levelstay{GPU Memory Management and Sharing}
GPU memory management is a well-known performance bottleneck in many applications and our system is no exception~\cite{vast} \jd{I found one here}. Particularly under high cache pressure, a significant fraction of time in our system goes to CUDA memory management routines. A more performant implementation would bypass these interfaces and instead provide a user-space memory allocator tuned to \system{} workloads (similar to PipeSwitch~\cite{pipeswitch}). Furthermore, the cache management policy itself can be better integrated with higher-level scheduling and fairness concerns. Since GPU workloads tend to have predictable data access patterns, we can use learned policies to decide which data objects to free or prefetch. Our current cache management policy exploits this to free ephemeral buffers (that are unlikely to be re-used) more aggressively than constant inputs.

\levelstay{Dynamic Graphs and Expressivity}
The current \system{} design only supports static graphs of CUDA kernels. This requirement is motivated by the need to limit host-side computation of arbitrary user code on the \system{} executor. However, some compromise may be possible. TVM supports a narrow language for describing dynamic graphs called relayIR~\cite{tvmRelay}. Richer semantics may also be possible for applications that perform a small amount of host-side computation to control GPU operation. These code snippets must be constrained in their scope. There are techniques to provide such constrained and safe code snippets going back to at least the 1970's~ \cite{deutschInformer} \np{there are obviously a ton of things here from DB UDFs to kernel modules to CDN stuff, not sure how much to look up and cite}.

==> mainSrc/conclusion.tex <==
Serverless computing is a wonderful thing; it simplifies programming at scale, drives higher resource utilization, and frees users from complex provisioning decisions. As expensive application accelerators like GPUs rise in importance in modern workloads, these properties are more important than ever. Simply adding GPUs to existing serverless techniques will not be sufficient; they are too different. In this paper, we presented \gls{kaas}, a truly serverless interface to GPUs that can integrate them naturally into the serverless ecosystem while preserving all the benefits we've come to know and love. \gls{kaas} frees users from tricky explicit allocations, effectively utilizes precious GPU resources in a multitenant environment, and frees system implementers to take full advantage of the unique properties of these devices. With \gls{kaas}, we were able to provide 50x higher throughput and 16x lower latency than \gls{faas} when the number of tenants exceeded available resources.

==> mainSrc/currentAproaches.tex <==
Today, GPUs are exposed to users through a number of allocation schemes. We present the most relevant approaches here (see Figure \ref{fig:gpuDeployments}).

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.37\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/serverful.pdf}
        \caption{Serverful}
        \label{fig:serverfulDeployment}
    \end{subfigure}
    \begin{subfigure}[b]{0.27\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/gpufaas.pdf}
        \caption{GPU+FaaS}
        \label{fig:gpufaasDeployment}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/kaas.pdf}
        \caption{KaaS}
        \label{fig:kaasDeployment}
    \end{subfigure}
    \caption{\textbf{Three possible GPU deployment strategies} In a serverful deployment, users get allocated a large collection of CPUs and GPUs for an unbounded period of time. In GPU+FaaS, users run a short stateless task that uses a small number of resources (e.g. a single GPU) only for the duration of the task. In \system{}, users submit CPU and GPU tasks separately where each task type runs in a resource-specific environment.}
    \label{fig:gpuDeployments}
\end{figure}


\subsection{Serverful}
Traditionally, GPUs have been deployed in a serverful manner as PCI-E attached cards in a virtual machine (Figure \ref{fig:serverfulDeployment}). Users are fully responsible for driving enough utilization to justify the added cost. This is challenging. Microsoft reports only 52\% average utilization of their deep learning GPUs~\cite{msGPUUtilization}. Importantly, the tight coupling of host and GPU resource allocations leads to wasted host resources as well. From the same trace, Microsoft reports only about 30\% utilization of CPUs for GPU-enabled deep learning jobs while memory utilization is well over 90\%. While the trace does not report total memory capacity, they report that 6.2\% of node failures are due to exceeding host memory capacity. It is challenging to predict memory and CPU requirements, necessitating wasteful overprovisioning to avoid failures.

\subsection{Service API}
Rather than exposing accelerators directly to users, some cloud systems expose \textit{services} that then utilize the accelerators. Of particular note is Microsoft's Catapult system that deploys FPGAs as network endpoints that can be programmed into ``FPGA Microservices''~\cite{catapult}. For example, the Microsoft Brainwave project places deep neural network models directly on a network of FPGAs that can be addressed from conventional software~\cite{brainwave}. However, Catapult is neither general purpose nor multi-tenant, limiting its deployment to internal tools or high-level customer-facing services~\cite{msCatapultProduct}. Other services focus on a narrow domain such as deep learning~\cite{clockwork,infaas,crankshaw2017clipper}. These services run on dedicated clusters with specialized schedulers and data management policies. They are not able to take advantage of the broader serverless infrastructure for scheduling, data movement, and end-to-end performance guarantees. This lack of generality and integration can lead to many of the challenges experienced by serverful approaches in a multitenant environment where workloads have a diversity of resource requirements.

\subsection{GPU Virtualization}
Traditional serverful approaches allocate one or more GPUs to clients persistently. This can be wasteful when applications cannot effectively use an entire GPU. The tight coupling of host and GPU resources can also lead to resource stranding where GPUs cannot be allocated to users due to insufficient host resources. One technique to avoid these issues is \emph{GPU Virtualization} where clients are allocated fractions of a GPU. On a single node, NVidia provides multi-process server (MPS) and multi-instance GPU (MIG) for this purpose~\cite{mig,mps}. API forwarding techniques like rCUDA or VMWare bitfusion additionally avoid stranding by allowing GPUs and hosts to be allocated from different physical servers~\cite{rcuda,bitfusion,juiceLabs}. While these techniques make resource allocation more flexible, they do not address the fundamental limitations of serverful approaches. GPUs are allocated persistently on a per-client basis regardless of client load. Host and GPU resource allocations also remain coupled. Indeed, GPU virtualization multiplies the number of host resources needed by increasing the number of supported GPU clients. These approaches also do not address broader distributed system concerns like scheduler integration or data layer management.

\subsection{FaaS+GPU}
Some systems have offered a more serverless FaaS+GPU approach. In these systems, users upload a CPU-oriented function and the provider ensures that the function runs in a container that includes a GPU (Figure \ref{fig:gpufaasDeployment})~\cite{ray,nuclio,openfaas,kimServerlessGpu}. While these approaches present a familiar interface to accelerators, they give away many of the features that make serverless appealing.

As an example, the Ray distributed computing framework supports GPU-enabled remote functions called \emph{tasks}, but requires that applications carefully design their tasks to manually share resources and clean up properly when they finish. In practice, this is difficult to achieve. Indeed, users are advised in the documentation to force Ray to restart workers on each task invocation to ensure resources are properly freed~\cite{rayWorkerKillDocs}. Rather than using serverless functions, users are often advised to fall back to non-serverless stateful actors to manually manage GPU resources.

Another challenge that arises with this approach comes from cold start mitigation strategies. CPU functions incur a significant startup latency due to container and language runtime initialization. A Python script that simply imports tensorflow and immediately exits takes \SI{1.9}{\second} when the OS buffer cache is warm. A true cold start that must read from disk takes even longer at \SI{6.8}{\second}\footnote{Run on an Amazon EC2 p3.2xlarge instance with a general-purpose SSD (gp2).}. To minimize the impact on users, cloud providers often keep function executors allocated in anticipation of a new request~\cite{msWarming}. This policy is reasonable because SMT threads are cheap and processes are easily idled. The same policy applied to a GPU would cost at least 60x more since the provider would need to keep the much more expensive GPU idle\footnote{Based on the capital costs of the 56 SMT core Xeon Platinum 8380 (\$10k MSRP\cite{xeonCost}) and an Nvidia A100 (\$12k\cite{a100Cost}).}. While the increased cost of a GPU is justified when fully utilized, both resources provide the same utility when idle: zero.

==> mainSrc/evaluation.tex <==
\levelstay{Experimental Setup}
Our experiments were performed on a single p3.8xlarge Amazon EC2 instance with 32 vCPUs and 4 Nvidia V100 GPUs (with \SI{16}{\giga\byte} of memory each).

\levelstay{Micro-Benchmarks}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figs/kaasBench.pdf}
%     \caption{Chained matrix multiply micro-benchmark. Each multiply has one constant matrix and one dynamic matrix. Dynamic inputs are preprocessed before being passed to the first layer. Each subsequent step uses the output of the previous layer. The initial input, constants, and final output are stored in the data layer while the intermediate matrices are ephemeral.}
%     \label{fig:kaasMicroBench}
% \end{figure}

For this analysis, we use a simple chained matrix multiplication micro-benchmark. Inputs are taken from the data layer and fed through a series of multiplications on the GPU before writing the final matrix output back to the data layer. Each multiplication uses a constant matrix that is read from the data layer but will not change between invocations (enabling caching). We configured the benchmark to use three layers with square matrices with a side length of 1024 single precision floats. The baseline \gls{gtask} implementation required the numpy, pickle, and pycuda python modules. For cold starts, the system has not seen any requests for the benchmark. For \glspl{gtask}, this means that it must create a new worker and initialize any python dependencies before running the \gls{gtask} code. For \glspl{ktask}, the system already has \gls{kaas} executors initialized since they are independent of any particular request. However, those executors must parse the request, link against the specified \gls{cuda} libraries, and load all data from the data layer. On warm starts, both task types already have a worker ready to execute the request immediately.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/microWarm.png}
        \caption{Warm Start}
        \label{fig:kaasMicroWarm}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/microCold.png}
        \caption{Cold Start}
        \label{fig:kaasMicroCold}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/microKaasOnly.png}
        \caption{\gls{kaas} Cold vs Warm Start}
        \label{fig:microKaasWarmCold}
    \end{subfigure}
    \hspace{0.07\linewidth}
    \begin{subfigure}[b]{0.35\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/microLegend.png}
        \vspace{0.8cm}
        \label{fig:kaasResLegend}
    \end{subfigure}
    \caption{\textbf{Microbenchmark Results} \emph{Kernel Run} is the time spent actually executing the request's kernels. \emph{Kernel Init} is the time to link any needed precompiled \gls{cuda} libraries. \emph{GPU Malloc} and \emph{GPU Copy} encompass all device data management while \emph{Data Layer} measures host data management. \emph{Overheads} measure any additional tasks performed by the worker including request parsing, worker initialization, and Ray framework overheads.}
    \label{fig:kaasMicro}
\end{figure}

Figure \ref{fig:kaasMicro} shows the results of this experiment. We begin by observing that \glspl{ktask} and \glspl{gtask} have similar warm-start performance (Figure \ref{fig:kaasMicroWarm}). This is not surprising as both implementations must perform the same steps. Any differences are mostly down to implementation details. Next, we move our attention to cold starts (Figure \ref{fig:kaasMicroCold}). Here we see the drastic impact of starting a new Python process for \glspl{gtask}. Even though the microbenchmark only imports a minimal set of packages, it still takes an additional \SI{400}{\milli\second} to load (a 46x increase). In contrast, the only cold-start overheads experienced by \glspl{ktask} come from warming the data caches with the constant matrices. To see this in more detail, Figure \ref{fig:microKaasWarmCold} compares warm and cold starts experienced by \glspl{ktask}. As expected, the time to load an additional three matrices adds significant time to both the data layer and GPU memory management phases, but there are no other overheads.

\levelstay{Multitenant Workload}
As we saw with the microbenchmarks, \glspl{ktask} behave similarly to \glspl{gtask} for a single warm workload. However, when there are multiple clients, the behavior changes dramatically. As discussed in \S\ref{sec:pool}, the \gls{gtask} approach requires a policy that assigns GPUs to workloads exclusively, falling back to terminating and restarting workers as the number of workloads exceeds the available GPUs. These cold starts prevent the system from fully utilizing its GPU resources. \gls{kaas}, in contrast, is able to share a limited pool of GPUs more effectively.

\begin{figure*}
    \centering
    \includegraphics[width=0.65\textwidth]{figs/expPipeline.png}
    \caption{\textbf{Multitenant Environment:} Clients submit requests over a ZeroMQ socket to a server that submits per-request \gls{func} pipelines to Ray. Each request pipeline involves optional CPU-only pre and post-processing steps with a GPU-based execution phase. The server proxies pipeline outputs back to the client.}
    \label{fig:expPipeline}
\end{figure*}

We now evaluate four real-world applications in a multi-tenant environment with two scenarios: online and offline. In the online scenario, we evaluate how the system supports latency-sensitive workloads like model serving or interactive data analytics where requests arrive according to a Poisson process. To understand sustained throughput, we evaluate an offline scenario where all workloads submit requests as fast as possible. Two of our workloads, resnet50 and BERT, are deep-learning inference workloads generated by the TVM interface. These workloads consist of many small kernels operating over many small buffers. Deep learning models also have significant data re-use through the model weights. The cGEMM workload is a chained complex number matrix multiply using our Cutlass library interface. It multiplies a large constant $10000\times25000$ matrix by a narrow $100\times10000$ matrix that changes on each invocation. Both contain \SI{32}{\bit} complex floats. This results in small inputs and outputs but a large amount of cacheable data. Finally, the Jacobi workload uses the low-level \gls{kaas} interface to implement an iterative solver using the Jacobi method~\cite{jacobiSource}. This workload uses \gls{kaas}'s iteration control-flow mechanism to run a fast update kernel for 3000 iterations. The input matrix contains $512\times512$ \texttt{float32s} and is accumulated into a $512\times1$ \texttt{float64} output. There is no data re-use between invocations. Table \ref{tbl:kaasWorkloads} summarizes the properties of these workloads.

% \begin{table}
% \centering
% \begin{tabular}{|l|l|l|l|l|}
%     \hline
%     \textbf{Name} & \textbf{Constant Mem} & \textbf{Dynamic Mem} & \textbf{GPU Time} & \textbf{Host Time} \\
%     \hline
%     resnet50 & \SI{129}{\mega\byte} & \makecell[l]{\SI{5.63}{\mega\byte} (TVM) \\  \SI{45.9}{\mega\byte} (KaaS)} & \SI{3.8}{\milli\second} & \SI{9.7}{\milli\second} \\
%     \hline
%     BERT & \SI{1.34}{\giga\byte} & \makecell[l]{\SI{6.33}{\mega\byte} (TVM) \\  \SI{1.89}{\giga\byte} (KaaS)} & \SI{91.8}{\milli\second} & \SI{132.0}{\milli\second} \\
%     \hline
%     cGEMM & \SI{2.00}{\giga\byte} & \SI{8.00}{\mega\byte} & \SI{38.8}{\milli\second} & \SI{0}{\milli\second} \\
%     \hline
%     Jacobi & \SI{0}{\mega\byte} & \SI{1.08}{\mega\byte} & \SI{52.1}{\milli\second} & \SI{0}{\milli\second} \\
%     \hline
% \end{tabular}
% \caption{End to end workload properties. For the dynamic memory of resnet50 and BERT, TVM implements buffer recycling while KaaS does not, so we provide the two different numbers for this category. See \S\ref{ch:log:kaas:tvm} for more details.}
% \label{tbl:kaasWorkloads}
% \end{table}

\begin{table}
\small
\centering
\begin{tabular}{|l|l|l|l|l|}
    \hline
     & \textbf{resnet50} & \textbf{BERT} & \textbf{cGEMM} & \textbf{Jacobi} \\
     \hline
     \makecell[l]{\textbf{Constant} \\ \textbf{Memory}} & \SI{129}{\mega\byte} & \SI{1.3}{\giga\byte} & \SI{2.0}{\giga\byte} & \SI{0}{\mega\byte} \\
     \hline
     \makecell[l]{\textbf{Dynamic} \\ \textbf{Memory}} & \SI{6}{\mega\byte} & \SI{6}{\mega\byte} & 
     \SI{8}{\mega\byte} & \SI{1}{\mega\byte} \\
     \hline
     \textbf{GPU Time} & \SI{4}{\milli\second} & \SI{92}{\milli\second} & \SI{39}{\milli\second} & \SI{52}{\milli\second} \\
     \hline
     \textbf{CPU Time} & \SI{10}{\milli\second} & \SI{132}{\milli\second} & \SI{0}{\milli\second} & \SI{0}{\milli\second} \\
     \hline
\end{tabular}
\caption{End to end workload properties.}
\label{tbl:kaasWorkloads}
\end{table}

In addition to the GPU-based \glspl{func}, the workloads also include pre and post processing \glspl{func} that occur exclusively on the host with no GPU requirements. These \glspl{func} form a graph that is lazily executed as inputs become available. Finally, this experiment uses multiple external clients that communicate with the Ray-based service through a network protocol using ZeroMQ~\cite{zmq}. Figure \ref{fig:expPipeline} shows the complete setup.

\leveldown{Offline Workloads}
We begin with a throughput-oriented scenario where workloads from many clients submit requests as quickly as possible with no regard for latency. In this case, we measure the aggregate throughput of the system. This indicates whether or not the GPU resources remain highly utilized as the number of clients increases.

Figures \ref{fig:throughputLowMem} and \ref{fig:throughputHighMem} show the results from this experiment. We see that \glspl{ktask} and \glspl{gtask} both perform well when there are sufficient GPU resources to support the workloads. However, as we exceed the number of available GPUs, the \gls{gtask} approach's throughput drops dramatically due to frequent worker cold starts. \glspl{ktask} do not suffer significant slowdowns as we exceed available GPUs because the system is able to handle requests from different clients without restarting the \gls{kaas} executor.

The \gls{ktask} implementation of cGEMM only begins to slow after about 20 replicas. This is the point at which we begin to exceed available GPU memory for cached weights and \gls{kaas} must begin evicting and re-loading constant buffers. Unlike the sharp performance drop seen with \glspl{gtask}, there is a more gradual performance impact with \glspl{ktask} since the cache can be managed at a fine granularity. Even at 32 replicas, we still see significantly higher throughput with \gls{kaas}. This comes down to the difference in cold-start behaviors between the two approaches. For \glspl{gtask}, the system must boot a fresh python process and initialize any packages and state needed to run the model, while \glspl{ktask} need only reload model weights from the host data cache.

Unlike cGEMM, resnet50 is a small model that fits easily within GPU memory. It experiences no significant slowdowns, even at 32 replicas. However, single-client warm-start performance is somewhat slower for \glspl{ktask} than the \gls{gtask} implementation. This is due to implementation differences between the two systems. The \gls{gtask} implementation uses TVM's highly optimized C++ runtime while \gls{kaas} uses a simple Python implementation. While these differences are easily amortized by the larger kernels used by BERT or cGEMM, resnet50 consists of many very small kernels that accentuate system overheads. Fundamentally, the same work is done in both implementations and a more optimized \gls{kaas} executor implementation should behave similarly to TVM.

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figs/throughputLowMem.png}
    \caption{\textbf{Aggregate throughput of low-memory workloads.} These workloads fit easily within GPU memory and see no aggregate throughput loss in \gls{kaas} as we increase the number of replicas. \gls{gtask} workloads require exclusive access to GPUs and must begin cold-starting workers after 4 replicas.}
    \label{fig:throughputLowMem}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.8\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/cdfBert4.png}
        \label{fig:bertCDF4}
    \end{subfigure}
    \begin{subfigure}[b]{0.8\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/cdfBert5.png}
        \label{fig:bertCDF5}
    \end{subfigure}
    \begin{subfigure}[b]{0.8\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/cdfBert16.png}
        \label{fig:bertCFG16}
    \end{subfigure}
    \caption{CDFs of BERT response latency for different numbers of replicas.}
    \label{fig:CDFRes}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figs/throughputHighMem.png}
    \caption{\textbf{Aggregate throughput of high-memory workloads.} These workloads consume a large amount of GPU memory. When the aggregate memory requirements exceed available GPU memory, \gls{kaas} must begin evicting and re-loading objects from the GPU memory cache. This leads to a gradual decline in performance as cache pressure increases.}
    \label{fig:throughputHighMem}
\end{figure}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.335\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/latDistResults_resnet50.png}
        % \vspace{-0.8cm}
        \caption{resnet50}
        \label{fig:latDistResnet}
    \end{subfigure}
    \hspace{2cm}
    \begin{subfigure}[b]{0.335\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/latDistResults_jacobi.png}
        % \vspace{-0.8cm}
        \caption{Jacobi}
        \label{fig:latDistJacobi}
    \end{subfigure}
    \begin{subfigure}[b]{0.335\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/latDistResults_bert.png}
        % \vspace{-0.8cm}
        \caption{BERT}
        \label{fig:latDistBert}
    \end{subfigure}
    \hspace{2cm}
    \begin{subfigure}[b]{0.335\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/latDistResults_cGEMM.png}
        % \vspace{-0.8cm}
        \caption{cGEMM}
        \label{fig:latDistCgemm}
    \end{subfigure}
    \caption{\textbf{Online benchmark results} The median response latency is plotted along with the 90th percentile tail.}
    \label{fig:latDistResults}
\end{figure*}

\levelstay{Online Workloads}
In this experiment, we simulate a latency-sensitive online environment using the MLPerf Inference load generator in server mode~\cite{mlperfinference}. Clients submit requests to the framework according to a Poisson process with their mean arrival rate set to 80\% of peak throughput (to ensure stability). We report the median and 90th percentile response latency for each configuration.

Figure \ref{fig:latDistResults} shows the results of this experiment. We see very similar behavior to the offline scenario. When the number of clients does not exceed available resources, both approaches behave reasonably well. However, when we exceed available resources, the \gls{gtask} approach is forced to cold-start new actors for nearly every request, resulting in very poor \gls{tail}. In effect, the \gls{tail} becomes a measure of cold start time. This latency depends primarily on the python dependencies and initialization tasks for each workload. \glspl{ktask} are able to effectively share GPUs, resulting in no significant impact on \gls{tail}, even as we exceed the number of available GPUs. However, the cGEMM \gls{ktask} begins to slow down after about 20 replicas as the aggregate constant memory exceeds GPU memory. Still, even at 32 replicas, the cGEMM \gls{ktask}'s \gls{tail} is far below the \gls{gtask} version due to the difference in cold start performance.


Figure \ref{fig:CDFRes} shows the CDFs of response latency at key points in the configuration space. Similar to Figure \ref{fig:latDistResults}, we configure the experiment to submit requests at 80\% of peak throughput to ensure queue stability. The maximum throughput of \glspl{gtask} is significantly lower than \glspl{ktask} so we plot CDFs for \glspl{ktask} at both an equivalent submission rate to \glspl{gtask}, and at peak \gls{ktask} throughput. At 4 replicas, each replica has a dedicated GPU. In this case, both \glspl{ktask} and \glspl{gtask} behave similarly with only minor differences due to implementation details. As we exceed 4 GPUs, the system must begin sharing GPUs between replicas. Even with only one extra replica, we see the \gls{gtask} \gls{tail} suffer significantly since replicas may need to evict an existing \gls{gtask} before cold-starting. As we increase the concurrency to 16 replicas, even the best 10th percentile latency suffers as replicas become nearly guaranteed to require a cold start. In contrast, \glspl{ktask} experience very consistent latencies as the number of replicas increase. Even at 16 replicas, there is no noticeable reduction in latency.

==> mainSrc/future.tex <==
\Gls{kaas} serves as a proof-of-concept for a larger vision of \emph{heterogeneous \gls{faas}}. In a heterogeneous \gls{faas} system, users design their application around a common data layer and function graph interface. However, the functions themselves can be implemented using any number of techniques. For example, some functions may want to take advantage of specialized unikernel operating systems while others may require more traditional full-featured containers~\cite{seuss}. As new specialized hardware technologies emerge, they can be integrated simply as a new function type. In fact, users or the serverless framework could decide between multiple implementations of the same functionality at runtime based on current system state as proposed by INFaaS~\cite{infaas}. Even though the functions themselves are implemented in radically different ways, the common execution framework means that applications do not need significant changes to use new technologies.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/pcsiGraph.png}
    \caption{\textbf{Hetergeneous function graph} While each function can be implemented in different ways, the general graph structure is common to all.}
    \label{fig:pcsiGraph}
\end{figure}

\levelstay{Serverless Accelerators}
FPGAs are an appealing target for serverless computing due to their high cost and ability to support diverse workloads. Microsoft has deployed FPGAs in their datacenters to support a wide range of workloads from deep learning to network function offload~\cite{catapult}. Ringlien, et al., propose ways that FPGAs could be made more multitenant~\cite{cloudFPGA}. As heterogeneous \gls{faas} becomes more common, we could envision \emph{serverless \glspl{soc}} that is optimized for \gls{kaas}-like systems. Since \gls{kaas} does not run user-provided code on the host, this serverless \gls{soc} would need only a low-power CPU and specialized protocol accelerators~\cite{sagarProtobuf,dagger}. Most of the power and area would be dedicated to the application accelerator. This could drastically improve power, cost, and deployment flexibility. These benefits have already been realized in the storage space~\cite{flashblade,pelican}. Microsoft's Catapult system and Google's TPU pods similarly demonstrate the potential benefits of resource-specific hardware platforms~\cite{tpupod,catapult}.

==> mainSrc/implementation.tex <==
We now present an implementation of \gls{kaas} using the Ray distributed computing framework~\cite{ray}. In addition to the core system, we provide a number of methods for users to implement \glspl{ktask}, including a TVM-based deep learning compiler, a pre-made BLAS library based on Nvidia Cutlass, and hand-written applications.

Throughout this section, we assume a scenario in which there are multiple \emph{clients} submitting requests for a particular \gls{func}. We use the term \emph{\gls{func}} to refer to a particular logical function, independent of any particular instantiation of that function. For simplicity, we assume clients send requests to only one \gls{func} and that different clients use different \glspl{func}.

\levelstay{Ray Implementation}
\label{ch:logLkaas:rayImplementation}

\leveldown{Ray Background}
Ray provides users with a Python \gls{api} to run stateless functions called \emph{tasks}, or stateful \emph{actors} across a cluster. Data are communicated using references to objects in an immutable object store called \emph{Plasma}. References are a form of \emph{future}~\cite{futures} and can be created before their associated object is available. Ray takes advantage of this to create lazily-executed graphs of tasks/actors that are scheduled only when their input references are available. Ray maintains a number of processes on each node called \emph{workers} that execute tasks and actors. A single worker may execute many tasks, but actors are always run on a dedicated worker. To control resource usage, users may annotate tasks or actors with resource requirements such as the number of GPUs required. Ray then ensures they are run on a worker that has been allocated those resources.

\levelstay{GPU-Enabled Functions in Ray}
Ray does not enforce isolation of resources for tasks. Instead, it relies on applications to ensure they do not exceed their limits. Furthermore, tasks running on the same worker share resources at a fine granularity and must ensure that all resources are freed before exiting. This is difficult to ensure in practice, so the Ray documentation recommends forcing worker restarts on every invocation of GPU-enabled tasks~\cite{rayWorkerKillDocs}.

Actors are persistent and run on dedicated workers. They are less sensitive to resource management concerns and can cache GPU state between invocations. However, there cannot be more GPU-enabled actors than available GPUs in the system and users must manually manage their actors to ensure that they do not exhaust available resources.

As a baseline, we enhance Ray with a new safe GPU-enabled task type called \gls{gtask}. \glspl{gtask} are written in Python in the same way as regular Ray actors and tasks. Unlike Ray native tasks, \glspl{gtask} run on a dedicated worker per task with exclusive control of a GPU. They can opportunistically cache state between invocations. However, because \glspl{gtask} have exclusive control of their GPU, the system may need to terminate them to free resources for new \glspl{gtask}. \glspl{gtask} provide an interface similar to many \gls{faas} platforms like AWS Lambda or Google Cloud Functions.

\levelstay{\gls{kaas} Implementation in Ray}
To implement \gls{kaas} in Ray, we provide an additional GPU-typed function called a \emph{\gls{ktask}}. \glspl{ktask} behave similarly to Ray's CPU-based tasks; they take in object references, output new references, and execute based on input availability. However, rather than providing Python source, \glspl{ktask} are defined by a request object consisting of an execution graph of kernels to invoke and buffer specifications describing input, temporary, and output buffers as well as literals for simple pass-by-value inputs.

\glspl{ktask} are run by an alternative worker implementation called the \emph{\gls{kaas} executor} (Figure \ref{fig:kaasImpleLow}). Much like regular workers, the \gls{kaas} executor is responsible for managing \gls{ktask} code and caching objects from the object store. A single executor can handle any \gls{ktask} without needing to restart. \glspl{ktask} are routed to \gls{kaas} executors based on a centralized scheduler that augments Ray's internal scheduler to consider input availability, data locality, and per-GPU load.

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/kaasImplLow.png}
    \caption{\textbf{Design of the KaaS executor} \gls{cuda} kernel code and a data cache are maintained on the host. The GPU maintains its own cache, independent of the host, and runs user kernels to completion in a \gls{cuda} stream.}
    \label{fig:kaasImpleLow}
\end{figure}

Internally, the \gls{kaas} executor manages code through a kernel cache that handles linking \gls{cuda} libraries and preparing kernels for invocation. Upon invocation, the linked kernel is launched using regular \gls{cuda} \glspl{api} on a single stream. Currently, kernels are invoked serially, though future implementations could support concurrent invocation of non-dependent kernels.

Data are managed through tiered host and GPU memory caches that extend Ray's built-in data layer. Objects are first loaded from Ray's object store into a data cache in host memory before being loaded into GPU memory. Ephemeral intermediate buffers are also cached in GPU memory to avoid frequent calls to \gls{cuda}'s expensive memory allocator. The current design is a hybrid inclusive/exclusive cache where inputs are kept in both host and GPU caches, but outputs and intermediates exist only in the GPU cache. When GPU memory capacity is exceeded, the GPU cache first evicts from the set of objects with only one use before considering more frequently used objects. Both sets use a least-recently-used policy.

\levelstay{GPU Worker Pool}
\label{sec:pool}
Both \glspl{ktask} and \glspl{gtask} require custom workers to run on each GPU. For \glspl{gtask}, these workers are user-defined actors. For \glspl{ktask}, this is the \gls{kaas} executor. We implemented a custom worker pool mechanism in Ray to manage the scheduling of these workers. The worker pool includes two scheduling policies:

\begin{itemize}
    \item \textbf{CFS-Affinity:} The CFS-Affinity policy is based on the completely fair scheduler from Linux~\cite{cfs} and ensures that clients get a fair share of GPU runtime. It allows client requests to run on any worker, but preferentially routes requests from the same client to the same GPU to maximize data locality. 

    \item \textbf{Exclusive:} The exclusive policy ensures that no two \glspl{func} run on the same worker, while repeated invocations of the same \gls{func} are always routed to the same set of workers. To maintain this property, the exclusive policy must kill existing workers to make room for new requests if the number of unique \glspl{func} exceeds the number of GPUs.
\end{itemize}

\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \includegraphics[width=0.7\linewidth]{figs/schedBalance.png}
        \caption{\textbf{CFS-Affinity Policy} Requests from any client can go to any GPU. Requests are processed according to the CFS algorithm, but priorities are weighted by a GPU affinity. In this scenario, the request from Client1 will be routed to GPU3.}
        \label{fig:schedAffinity}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \includegraphics[width=0.6\linewidth]{figs/schedExclusive.png}
        \caption{\textbf{Exclusive Policy} There must be a client-specific worker on each GPU. Clients 0 and 2 have pools of GPUs assigned to them while Client 1 currently has no assigned GPUs. In this scenario, the exclusive policy would need to re-balance the pools, taking GPU3 from Client 2 and cold-starting a worker for Client 1 on it.}
        \label{fig:schedExclusive}
    \end{subfigure}
    \caption{\textbf{\gls{kaas} Schedulers:} In this scenario, clients are submitting a series of requests for a client-specific \gls{func}. there are three independent clients and four GPUs. GPUs $0-2$ are currently running requests. GPU3 was previously running a request from Client 2 but is now idle.}
    \label{fig:kaasSched}
\end{figure*}

The CFS-Affinity policy, depicted in Figure \ref{fig:schedAffinity} launches a worker on each GPU at boot time and never restarts them. Client requests share the same workers (e.g. the \gls{kaas} executor). It maintains a running count of each client's accumulated GPU time weighted by GPU affinity. For non affinitized GPUs, the client's runtime is penalized by 10x their average request latency. When a GPU becomes idle, the scheduler searches the clients for the one with the smallest weighted runtime to run. This algorithm ensures that all clients receive similar GPU time while remaining work-conserving. By attempting to route requests to the same GPU when possible, it maximizes data locality in GPU memory. \gls{kaas} can safely use the CFS-Affinity policy because the permanent worker is the \gls{kaas} executor which can service requests from multiple \glspl{ktask} without needing to restart. \glspl{gtask} require strict isolation between workers and cannot use this policy.  

The Exclusive policy in Figure \ref{fig:schedExclusive} is more complex. It must ensure that requests always run on a dedicated per-client worker rather than sharing a GPU execution environment. To do this, the Exclusive policy maintains independent per-client \emph{pools} of workers. These pools route requests from a single client to the next available GPU in the pool. If a client submits a request that cannot be serviced from its pool immediately, the policy may consider shrinking an existing pool to free GPU resources for the new request. It begins by finding the largest pool to use as an eviction candidate $p_{victim}$. If there are multiple pools with the largest size, the least-recently evicted pool is chosen. If the requesting client's pool, $p_{req}$, is smaller than $p_{victim}$, the algorithm will evict a GPU from $p_{victim}$ and assign it to a new worker in $p_{req}$. If $p_{victim}$ has idle GPUs, they are simply re-assigned to $p_{req}$. Otherwise, the algorithm selects a busy GPU and waits for the currently executing request to finish before re-assigning the GPU to $p_{req}$. If $p_{req}$ is in the set of largest pools, the algorithm simply blocks the request until a worker from $p_{req}$ becomes available. We use the Exclusive policy for all \gls{gtask} experiments.

\levelup{Application Support}
\label{sec:appSupport}
\leveldown{Low-Level API}
\label{sec:kaasApi}
\Gls{kaas} exposes a python \gls{api} for describing \gls{ktask} requests. Figure \ref{fig:api} shows the datastructures used to describe \glspl{ktask}. These requests consist of a list of kernels to invoke and their associated inputs, outputs, and temporary buffers. Kernels may also take literal arguments that are passed by value in the \gls{kaas} request. The kernels themselves are described using a filesystem path to the compiled \gls{cuda} code and a kernel name within that file along with the appropriate \gls{cuda} grid and block dimensions to use when launching. In addition to kernels, we provide a simple control-flow mechanism for fixed-length iteration. These requests are then serialized by Ray and sent to the \gls{kaas} executor for processing. Callers immediately receive a reference to the future response, just like any other Ray task.

\gls{ktask} inputs are passed as Ray object references, while output references are provided in the \gls{ktask} return value. Internal buffers are only valid for the duration of the request and are not associated with the Ray object store. Upon completion of the request, any output buffers are written back to the Ray object store and a reference to this output is returned to the caller.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/apiTables.png}
    %\includegraphics[width=0.8\linewidth]{figs/exampleReq.pdf}
    \caption{Low-level \gls{kaas} \gls{api}. \glspl{ktask} are described by a \texttt{kaasReq} data structure that contains a list of CUDA kernels to run and their arguments. Arguments can either be objects in the object store or passed by value as literals.}
    \label{fig:api}
\end{figure}

\levelstay{TVM-Based Deep Learning Compiler}
\label{sec:tvm}
Rather than manually writing \glspl{ktask}, users can generate \glspl{ktask} using high-level frameworks and compilers. We modified the TVM deep-learning compiler to include \gls{kaas} as a backend target~\cite{tvm}. While we chose TVM for our prototype, \gls{kaas} can behave as a backend to any deep learning framework that generates static graphs of \gls{cuda} kernels. At a high level, TVM functions by generating a DAG of operators to execute the model. Each of these operators consist of one or more \gls{cuda} kernels. This scheme has a 1-1 correspondence with \gls{kaas} graphs, with the only difference being that each operation needs to be expanded into one or more kernel nodes.

Our approach to converting the TVM runtime graph to a \gls{ktask} is straightforward. First, we use TVM to generate the \gls{cuda} kernel library and the static runtime graph. We then extract the necessary information, such as the grid and block dimensions for each kernel. This information is then used to generate the \gls{kaas} code for the request.

\levelstay{BLAS Library}
\label{sec:cutlass}
The \gls{cuda} ecosystem has benefited greatly from high quality libraries of common kernels such as cuBLAS and cuDNN~\cite{cublas,cudnn}. These libraries are often authored by service providers or device manufacturers. Likewise, we expect a similar ecosystem would grow around a realistic \gls{kaas} deployment. For this project, we ported one such library based on Nvidia's Cutlass BLAS library~\cite{cutlass}. Cutlass is a C++ template library that allows users to instantiate handles to specialized linear algebra kernels. We provide a \gls{kaas} interface to Cutlass through built in functions. Rather than uploading specific kernels, users can simply reference one of the system-provided functions. \gls{kaas} then manages interfacing with the library and managing device resources as needed.

While porting Cutlass to \gls{kaas} was non-trivial, it was a one-time cost borne by the system provider rather than individual users.

==> mainSrc/intro.tex <==
Resource utilization is a critical requirement in cloud computing. For users, this means minimizing costs by allocating only what they need while scaling up and down quickly. For cloud providers, this means being able to quickly reclaim idle resources that can then be rented to other customers. Serverless computing helps achieve these goals by focusing on time-bounded invocations of \emph{functionality} rather than explicit \emph{allocation} of resources. In other words, users ask for some function or service to be invoked without considering how or where it will run. In the case of function-as-a-service (FaaS), this functionality takes the form of small stateless functions written in general-purpose languages like Python or Javascript. 

Serverless computing has already seen significant adoption. Users get true pay-per-use and providers can quickly reallocate resources to other jobs. However, today's \gls{faas} systems remain narrow in scope by focusing on CPU-based workloads running general purpose code on familiar OS environments. To date, none of the major cloud providers offer a GPU-enabled \gls{faas} service. This is somewhat surprising given the growing popularity of application accelerators. Why is it challenging to deploy accelerators like GPUs in a \gls{faas} system? The problem lies in the techniques that make \gls{faas} practical to implement. \gls{faas} functions are small and limited in scope, they consume few resources when not executing, and use easily shared and subdivided resources. Providers are free to kill \gls{faas} containers as needed to free resources, or aggressively cache them to reduce cold starts. Furthermore, providers can mitigate the performance costs of explicit state by maintaining shared caches of their data layer. GPUs upend these assumptions. Unlike CPUs, GPUs are expensive, difficult to share on a fine granularity, and have their own memory that must be managed by the user.

This is not to say that GPUs are fundamentally incompatible with the \gls{faas} model; they simply require different techniques. Unlike general-purpose code, GPU functions (called \emph{kernels}) have limited capabilities and few dependencies which greatly simplifies function startup. GPU functions also have more predictable inputs and outputs, enabling greater optimizations from the \gls{faas} scheduler and data layer.

In this paper, we present a truly serverless interface to GPUs, called \gls{kaas}, that is able to take advantage of these properties to enable high-utilization of GPUs in the cloud with minimal performance overheads. In \gls{kaas}, GPUs become first-class citizens that are directly invoked through a GPU-specific function type (see Figure \ref{fig:kaasDagHigh}). Rather than explicitly mixing host and device code, users register \gls{cuda} kernels that run independently with no user-provided host code. Since the \gls{kaas} system is in full control of the GPUs, it is able to explicitly manage device memory and multiplex kernels from many users at a fine granularity.

For compute-heavy tasks, \gls{kaas} experiences virtually no decrease in aggregate performance, even when there are far more users than available GPUs. For memory-heavy workloads, \gls{kaas} performance degrades gracefully when GPU memory requirements exceed capacity. In our evaluation, we compare \gls{kaas} to a traditional \gls{faas} approach that allocates GPUs exclusively to functions during execution. Our results demonstrate 50x higher throughput and 16x lower latency for a compute-intensive linear system solver when the number of clients exceeds available GPUs by 4x. Even when total available GPU memory is exceeded by 1.5x, \gls{kaas} supports 53x greater throughput and 12.6x lower latency for a memory-intensive deep-learning inference benchmark.

We present the following key contributions:
\begin{itemize}
    \item A new GPU-native serverless function type, \gls{ktask}, that treats GPUs as first-class citizens.
    \item Three programming interfaces to \gls{kaas} functions: a low-level \gls{api}, a TVM-based compiler, and a suite of built-in libraries.
    \item Two scheduling algorithms that take advantage of the unique properties of \gls{faas} and \gls{kaas} functions.
    \item A Ray-based prototype of \gls{kaas} with drastically improved utilization of GPU resources in a multitenant environment.
\end{itemize}
\glsreset{ktask}

In \S\ref{sec:currentAproaches}, we discuss how GPUs are deployed today. \S\ref{sec:kaas} presents the \gls{kaas} programming model while \S\ref{sec:implementation} describes our Ray-based prototype. In \S\ref{sec:evaluation}, we evaluate this prototype against a traditional mixed host/GPU approach with a diverse set of applications ranging from deep neural-network model serving to general purpose linear algebra. We compare our work to other approaches to multitenant GPU utilization in \S\ref{sec:related}. We conclude in \S\ref{sec:future} with a discussion of how the \gls{kaas} model can be extended to new resource types and enable new technologies. 

% However, today's FaaS systems largely focus on CPU-based workloads. To date,
% none of the major cloud providers offer a GPU-enabled FaaS service. This is
% somewhat surprising given the growing popularity of application accelerators.
% Why is it challenging to deploy accelerators like GPUs in a FaaS system? The
% problem lies in the techniques that make FaaS practical to implement. FaaS
% functions are small and limited in scope, they consume few resources when not
% executing, and use easily shared and subdivided resources. Providers are free to
% kill FaaS containers as needed to free resources, or aggressively cache them to
% reduce cold starts. Furthermore, providers can mitigate the performance costs
% of requiring functions to explicitly store state by maintaining shared caches of their data layer. GPUs upend these assumptions. Unlike CPUs, GPUs are expensive, difficult to
% share on a fine granularity, and have their own memory that must be managed by
% the user.

% This is not to say that GPUs are fundamentally incompatible with the FaaS model; they simply require different techniques. Unlike general-purpose code, GPU functions (called ``kernels'') have far fewer dependencies and limited capabilities which greatly simplifies function startup. GPU functions also have more predictable inputs and outputs, enabling greater optimizations from the FaaS scheduler and data layer. 

% In this paper, we present a truly serverless interface to GPUs, called \System{} (\system{}), that is able to take advantage of these properties to enable high-utilization of GPUs in the cloud with minimal performance overheads. In \system{}, GPUs become first-class citizens that are directly invoked like any other cloud function (see figure \ref{fig:kaasDagHigh}). Rather than explicitly mixing host and device code, users register CUDA kernels that run independently with no user-provided host code. Since the FaaS system is in full control of the GPUs, our system is able to explicitly manage device memory and multiplex kernels from many users at a fine granularity.

% For compute-heavy tasks, we see virtually no decrease in aggregate performance, even when there are far more users than available GPUs. For memory-heavy workloads, \system{} performance degrades gracefully when GPU memory requirements exceed capacity. In our evaluation, we compare \system{} to a traditional FaaS approach that allocates GPUs exclusively to functions during execution. Our results demonstrate 50x higher throughput and 16x lower latency for a compute-intensive linear system solver when the number of clients exceeds available GPUs by 4x. Even when total available GPU memory is exceeded by 1.5x, \system{} supports 53x greater throughput and 12.6x lower latency for a memory-intensive deep-learning inference benchmark.

% In this paper, we present the following key contributions:
% \begin{itemize}
%     \item A new GPU-native serverless function type, \System{} (\system{}), that treats GPUs as first-class citizens in serverless applications.
%     \item Three core programming interfaces to \system{} functions; a low-level API, a TVM-based compiler, and a suite of built-in libraries.
%     \item Three distinct scheduling algorithms that take advantage of the unique properties of FaaS and \system{} functions.
%     \item A Ray-based prototype of \system{} with drastically improved utilization of GPU resources in a multitenant environment.
% \end{itemize}

% In \S\ref{sec:currentAproaches}, we discuss how GPUs are deployed today. \S\ref{sec:kaas} presents the \system{} programming model while \S\ref{sec:implementation} describes our Ray-based prototype of such a system. In \S\ref{sec:evaluation} we evaluate this prototype against a traditional mixed host/GPU approach with a diverse set of applications ranging from deep neural-network model serving to general purpose linear algebra. We conclude with a discussion of related work (\S\ref{sec:related}), and future research opportunities enabled by our system (\S\ref{sec:future}).

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\columnwidth]{figs/kaasDagHigh.pdf}
%     \caption{Serverless graph including both GPU and CPU-typed functions. While different function types have different implementations, at the application graph level they all behave similarly; they take inputs, perform computation, and produce outputs.}
%     \label{fig:kaasDagHigh}
% \end{figure}

==> mainSrc/kaas.tex <==
Fundamentally, existing approaches struggle because they cede control of GPUs to applications by tightly coupling host and GPU code. We take a different approach, called \glsentrydesc{kaas} (\gls{kaas}), that explicitly decouples host functions from GPU kernels at the system level (Figure \ref{fig:kaasDeployment}). Following the principles of serverless computing, our system takes user descriptions of GPU \emph{functionality} rather than providing GPU \emph{allocations}. This puts the responsibility for GPU memory management and scheduling on the system rather than relying on users to make optimal use of these expensive resources.

This strategy elevates GPU functionality to a first-class entity, along with traditional FaaS functions and other serverless services (see Figure \ref{fig:kaasDagHigh}). We refer to CPU-specialized functions as \glspl{ctask} and GPU-specialized functions as \glspl{ktask}. Rather than providing a Python source file or Linux container, \glspl{ktask} take the form of a graph of \gls{cuda} kernels to be executed. Graph inputs and outputs are provided as objects in the system data layer (e.g., keys in a key-value store). Other buffers like intermediate outputs and temporary buffers are described simply by their size. The system is then responsible for ensuring that all required buffers are available in GPU memory before beginning execution of the kernel graph. \glspl{ktask} are not permitted to dynamically allocate memory or access the data layer, leading to highly predictable resource requirements. Furthermore, \glspl{ktask} do not include any host code whatsoever, which simplifies the software environment on \gls{kaas} executors and prevents external side effects.

\begin{figure*}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{figs/kaasDagHigh.png}
        \caption{Serverless graph including both GPU and CPU-specialized tasks. While different task types have different implementations, at the application graph level they all behave similarly; they take inputs, perform computation, and produce outputs.}
        \label{fig:kaasDagHigh}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{figs/kaasDagLow.png}
        \caption{\glspl{ktask} are defined as a dataflow graph of individual \gls{cuda} kernels with predefined inputs, outputs, and temporary buffers. Inputs and outputs go through the data layer of the broader serverless infrastructure.}
        \label{fig:kaasDagLow}
    \end{subfigure}
    \caption{KaaS introduces a new GPU-specialized function type called a \gls{ktask}.}
    \label{fig:kaasDag}
\end{figure*}

\levelstay{Why KaaS?}
\gls{kaas} provides a number of important benefits over more traditional approaches to GPU multitenancy. Figure \ref{fig:featureGrid} summarizes these properties. The \gls{kaas} approach only explicitly uses GPUs in its programming, and presumably billing, model. This \emph{on-demand} allocation means that users are charged only for the time their code actually ran on the GPU rather than paying for long lived allocations. Users also do not need to allocate an entire server or VM just to use its GPUs. In serverful approaches like GPU virtualization, the user must pay for idle CPU, memory, and disk resources while the GPU is running. They must also explicitly manage resource deployment and scaling. While service APIs free users from resource allocation concerns, they exist in application-specific environments that do not share the data and scheduling semantics of general purpose serverless frameworks. \Gls{kaas} supports arbitrary GPU applications in a way that integrates natively with general-purpose serverless frameworks while allocating GPU resources to users only when needed.


\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/featureGrid.png}
    \caption{\textbf{Features of GPU multitenancy approaches} \emph{General purpose} systems can run arbitrary GPU code rather than focusing on a specialized domain. Systems that \emph{allocate GPUs on-demand} support pay-per-use, transparent autoscaling, and do not couple GPU allocation lifetimes with other resources. Finally, multi-tenant GPU systems can \emph{integrate natively} into a broader general-purpose serverless environment.}
    \label{fig:featureGrid}
\end{figure}

\levelstay{KaaS Interface}
\glspl{ktask} appear to the rest of the system like any other function. They provide named functionality without any explicit resource allocation, and interact with a common data layer for inputs and outputs.  While the \gls{kaas} approach is not tied to any specific serverless framework, it does assume a graph of functions communicating through a common data layer. Figure \ref{fig:kaasDagHigh} depicts a typical application in such a system. Each node in this graph can be implemented in many different ways, and node implementations can be modified or replaced without affecting the rest of the application. While this project focuses on GPU-typed functions, the \gls{kaas} approach can be applied to other function types such as deep learning-specific accelerators and specialized \glspl{soc}. We explore this in more detail in \S\ref{sec:future}.

While the external interface is assumed to be common to all function types, their internal implementation can be specialized. Figure \ref{fig:kaasDagLow} depicts the user's view of a \gls{ktask}. Users register a library of precompiled \gls{cuda} kernels that can then be combined into an execution graph when invoked. These kernels can come from common highly optimized libraries like NVidia's Cutlass linear algebra library~\cite{cutlass}, code compiled by frameworks like TVM~\cite{tvm}, or custom application-specific kernels. Each kernel is provided a set of GPU memory addresses representing inputs, temporaries, and outputs. These data objects are identified using the global data layer's semantics. Users may optionally specify a fixed number of iterations for a particular request. Future work will allow for more dynamic control flow similar to TVM's Relay IR or Dandelion's EDGE graph representation~\cite{tvmRelay,dandelion}.

\leveldown{Nearest-Neighbors Example}
We now describe an example \gls{ktask}: $N$ nearest neighbors. In this algorithm, we iteratively multiply an adjacency matrix $A$ by a vector $X$ representing starting vertices. On each iteration, the set of visited vertices in this iteration is accumulated into a vector $V$ representing the set of nearest neighbors. Algorithm \ref{eq:nearestNeighbor} describes this more formally.

\begin{algorithm}
\caption{An iterative $N$ nearest neighbors search over an adjacency matrix $A$. $X_1$ contains an initial set of vertices while $V_{N+1}$ contains the final set of nearest neighbors.}
\begin{algorithmic}[1]
\For{$i\gets 1, N$}
\State $X_{i+1}\gets A \cdot (X_{i} - V_i)$
\State $V_{i+1}\gets V_i+X_{i}$
\EndFor
\end{algorithmic}
\label{eq:nearestNeighbor}
\end{algorithm}

Figure \ref{fig:kaasNearestNeighbor} shows how this algorithm could be implemented in \gls{kaas}. The $A$ matrix along with an initial set of starting vertices $X_{inp}$ are passed in as objects in the data layer. Since $A$ is large and constant, it can be cached by the \gls{kaas} executor in GPU memory while the smaller $X_{inp}$ may change on each invocation. Some buffers like $X_{tmp}$ and $X_{iter}$ represent intermediate values and can simply be allocated by the \gls{kaas} executor. Finally, $V_{iter}$ represents an output of the system and will be written back to the key specified in the \gls{kaas} request. The kernels $vsub$, $vadd$, and $matmul$ can be implemented in a number of ways, including user-provided code or a built in and optimized library like graphBLAS~\cite{graphBLAS}. Users would likely call this function as part of a larger application with potentially long gaps between invocations. Unlike traditional approaches, users would not need to explicitly provision GPUs in their system and would only pay for the time the GPUs were actually running. In between user requests, the \gls{kaas} system would be free to execute functions from other users.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/NNGraph.png}
    \caption{\textbf{\gls{kaas} graph of a nearest neighbors algorithm (Equation \ref{eq:nearestNeighbor})} $X_{inp}$ and $A$ are read from the system data layer, while $V_{iter}$ will be written back as an output. $X_{tmp}$ and $X_{iter}$ are ephemeral buffers that will never be copied off the GPU.}
    \label{fig:kaasNearestNeighbor}
\end{figure}

\levelstay{Challenges}
These benefits do not come for free. The \gls{cuda} ecosystem has evolved around a model of locally-attached GPUs. Even multi-GPU workloads require host involvement to manage data transfers and scheduling. These assumptions are often baked into highly-tuned, but opaque, libraries. The \gls{kaas} model upends many of these assumptions. Additionally, placing GPUs behind a distributed abstraction will lead to additional invocation latency. Applications that finely interleave host and device code may not be able to amortize this additional latency.

The rise of serverless computing and modern machine learning frameworks suggests a promising path out of these challenges. Users have shown a willingness to decouple applications further in cloud applications, and backwards compatibility often takes a backseat to agility. The widely-adopted microservice architecture provides a good example of this~\cite{balalaie2016microservices}. These systems are a radical departure from traditional monolithic designs but enable rapid development, flexible deployment, and organizational flexibility. Another important trend is the rise of GPU-enabled application frameworks~\cite{tvm,tensorflow,pytorch,halide}. Many GPU applications, and deep learning in particular, are no longer interacting with the GPU directly. Instead, these applications are increasingly relying on frameworks and libraries to generate GPU code transparently. In many cases, these frameworks already support, and optimize for, remote execution. \gls{kaas} can leverage these trends to make radical changes to accelerator interfaces with minimal impact on users.

==> mainSrc/relatedWork.tex <==
The need to share and manage accelerators in a distributed system is not a new one. In \S\ref{sec:currentAproaches} we covered several broad categories of techniques to achieve this. In this section, we briefly cover several specific approaches.

\levelstay{Single GPU Sharing}
There are a number of techniques for sharing an individual GPU among multiple processes. Nvidia GPUs support multiple forms of sharing including \gls{cuda} contexts, Multi-Process Server (MPS), or Multi-Instance GPU (MIG)~\cite{mps,mig}. \gls{cuda} contexts allow sharing but do not enforce resource usage limits. MPS and MIG provide static allocations of resources from a particular physical GPU to processes. Techniques like r\gls{cuda} are similar to MPS or MIG but proxy requests across a network to a remote GPU~\cite{rcuda,juiceLabs}. In all cases, individual clients are assigned a specific GPU resource and must manage their own GPU resources explicitly for the lifetime of their allocation. While sharing increases the number of supported clients, those clients are still responsible for driving utilization of their allocation. The clients also require host CPU and memory resources, even if they are completely GPU bound. As the number of clients increase, CPU and memory underutilization can become significant. \Gls{kaas} allows for flexible run-time resource allocations and integrates the serverless data layer into GPU memory allocations. Client code can run on any available physical GPU in the system on a per-request granularity without user intervention. \az{One thing we can add here is how we solved rCUDA's usability problem with the TVM compiler and standard library.}

\levelstay{Domain Specific Systems}
Some domain-specific services, particularly for deep learning applications, are able to share accelerators among multiple clients. Google Cloud's TPU interfaces decouple TPU devices from host servers and manage communication and allocation. However, applications are still assigned specific devices for their lifetime and are responsible for driving adequate utilization~\cite{tpupod}.

RAMMER is a deep learning compiler and associated runtime that improves device utilization by abstracting deep learning models and accelerators into finer grained components and optimizing their scheduling~\cite{rammer}. \gls{kaas} applications also provide graphs of \gls{cuda} kernels which could be further optimized by systems like RAMMER.

PipeSwitch~\cite{pipeswitch} and Salus~\cite{salus} are two frameworks to facilitate sharing of a GPU between multiple cooperating deep learning processes on a single node. Like \gls{kaas}, they abstract GPU resources by handling memory allocation and kernel scheduling for the clients. Unlike \gls{kaas}, PipeSwitch still allows direct GPU access from host applications and requires applications to cooperate. Salus is more similar to the \gls{kaas} executor because it accepts graphs of kernel requests and associated memory needs. Neither system integrates into a larger serverless environment, requiring a strong association between host process and server/GPU. \Gls{kaas} allows for higher-level resource allocation/de-allocation and co-scheduling of traditional serverless functions, \glspl{ktask}, and data movement.

There are also a number of systems specifically tailored to deep learning inference (\cite{infaas,clockwork}) or training (\cite{gandiva}). These systems exploit the unique properties of deep learning, as well as cooperation from deep learning frameworks, to drive utilization and performance. Unlike these systems, \gls{kaas} is a general purpose serverless GPU interface for mutually unaware clients. It integrates natively into a broader general-purpose compute environment.
